ReSIFT: Reliability-Weighted SIFT-based Image Quality Assessment

This paper presents a full-reference image quality estimator based on SIFT descriptor matching over reliability-weighted feature maps. Reliability assignment includes a smoothing operation, a transformation to perceptual color domain, a local normalization stage, and a spectral residual computation with global normalization. The proposed method ReSIFT is tested on the LIVE and the LIVE Multiply Distorted databases and compared with 11 state-of-the-art full-reference quality estimators. In terms of the Pearson and the Spearman correlation, ReSIFT is the best performing quality estimator in the overall databases. Moreover, ReSIFT is the best performing quality estimator in at least one distortion group in compression, noise, and blur category.

==> Preprint for Arxiv/tab_param.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[htbp!]
\scriptsize
\centering
\vspace{-4.0mm}
\caption{List of the parameters and their values in ReSIFT}
\label{tab_param}
\begin{tabular}{lcc}
\hline
\textbf{Section/Block}                      & \multicolumn{1}{l}{\textbf{Parameter}} & \multicolumn{1}{c}{\textbf{Value}}                                                \\ \hline
\multirow{2}{*}{2.2. Low-pass filtering} & $f_{size}$                              & 4                                                                                  \\ 
                                         & $f_{\sigma}$                            & 5                                                                                  \\ \hline
\multirow{5}{*}{2.3. Color space transformation} & \multirow{2}{*}{$\kappa$}               & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}903.3\\ CIE standard\end{tabular}}      \\
                                         &                                         &                                                                                    \\  
                                         & $\epsilon$                              & 0.008856                                                                           \\  
                                         & \multirow{2}{*}{$M$}                    & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Adobe RGB  \\ stand. 1998\end{tabular}} \\
                                         &                                         &                                                                                    \\ \hline
2.4. Local normalization                 & $W$                                     & 20                                                                                 \\ \hline
\multirow{3}{*}{2.5. Spectral residual}  & $g_{size}$                              & 3                                                                                  \\  
                                         & $h_{size}$                              & 10                                                                                 \\  
                                         & $h_{\sigma}$                            & 3.8                                                                                \\ \hline
2.8. Descriptor matching                    & $thresh$                                & 1.4                                                                                \\ \hline
2.9. Percentile pooling                  & $perc$                                  & 5                                                                                  \\ \hline
\multirow{2}{*}{2.10. Nonlinear mapping} & $C_1$                                   & 100,000                                                                            \\ 
                                         & $C_2$                                   & 0.01                                                                               \\ \hline
\end{tabular}
\vspace{-6.0mm}
\end{table}

==> Preprint for Arxiv/tab_results.tex <==
\begin{table*}[]
\scriptsize
\centering
\caption{Performance of the IQA metrics based on Spearman correlation}
\label{tab_results}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline


\multirow{4}{*}{\bf Distortion Types} & \multirow{4}{*}{\bf Databases} & \multicolumn{5}{c|}{\multirow{2}{*}{\bf Pearson Correlation}}                                                            & \multicolumn{5}{c|}{\multirow{2}{*}{\bf Spearman Correlation}}                                                            \\
                  &                   & \multicolumn{5}{l|}{}                                                                             & \multicolumn{5}{l|}{}                                                                             \\ \cline{3-12} 
                  &                    & \multirow{2}{*}{\bf PSNR-HMA} & \multirow{2}{*}{\bf SR-SIM} & \multirow{2}{*}{\bf PerSIM} & \multirow{2}{*}{\bf SIFT} & \multirow{2}{*}{\bf Proposed} & \multirow{2}{*}{\bf IW-SSIM} & \multirow{2}{*}{\bf FSIM} & \multirow{2}{*}{\bf PerSIM} & \multirow{2}{*}{\bf SIFT} & \multirow{2}{*}{\bf Proposed} \\
                  &                   &                   &                   &                   &                   &                   &                   &                   &                   &                   &                   \\ \hline

\multirow{4}{*}{{\bf Compression}}   & {\bf Jp2k {[}LIVE{]}}           &0.982&0.957&0.976&0.966&0.000&0.979&0.981&0.977&0.959&0.000          \\ \cline{2-12} 
                                     & {\bf Jpeg {[}LIVE{]}}           &0.972&0.950&0.959&0.967&&0.960&0.962&0.958&0.948&       \\ \cline{2-12} 
                                     & {\bf Compression {[}TID13{]}}   &0.969&0.970&0.965&0.906&&0.937&0.960&0.963&0.888& \\ \cline{2-12} 
                                     & {\bf Blur-Jpeg {[}MULTI{]}}     &0.838&0.904&0.864&0.845&&0.869&0.854&0.812&0.893& \\ \hline
\multirow{3}{*}{{\bf Noise}}         & {\bf Wn {[}LIVE{]}}             &0.985&0.974&0.968&0.982&&0.980&0.979&0.991&0.975&\\ \cline{2-12} 
                                     & {\bf Blur-Noise {[}MULTI{]}}    &0.803&0.871&0.839&0.768&&0.893&0.864&0.818&0.903&\\ \cline{2-12} 
                                     & {\bf Noise {[}TID13{]}}         &0.907&0.894&0.903&0.746&&0.856&0.887&0.924&0.721&\\ \hline
\multirow{2}{*}{{\bf Communication}} & {\bf FF {[}LIVE{]}}             &0.954&0.943&0.946&0.946&&0.967&0.970&0.945&0.925&\\ \cline{2-12} 
                                     & {\bf Communication {[}TID13{]}} &0.800&0.905&0.854&0.793&&0.870&0.895&0.865&0.846&\\ \hline
\multirow{4}{*}{{\bf Blur}}          & {\bf GBlur {[}LIVE{]}}          &0.950&0.949&0.967&0.973&&0.983&0.983&0.973&0.961&\\ \cline{2-12} 
                                     & {\bf Blur {[}TID13{]}}          &0.931&0.959&0.935&0.892&&0.932&0.947&0.949&0.857&\\ \cline{2-12} 
                                     & {\bf Blur-Jpeg {[}MULTI{]}}     &0.838&0.904&0.864&0.845&&0.869&0.854&0.812&0.893&\\ \cline{2-12} 
                                     & {\bf Blur-Noise {[}MULTI{]}}    &0.803&0.871&0.839&0.768&&0.893&0.864&0.818&0.903&\\ \hline
{\bf Color}                          & {\bf Color {[}TID13{]}}         &0.814&0.672&0.800&0.663&&0.233&0.240&0.762&0.307&\\ \hline
{\bf Global}                      & {\bf Global {[}TID13{]}}     	   &0.762&0.571&0.585&0.075&&0.452&0.441&0.408&0.104&\\ \hline
{\bf Local}                          & {\bf Local {[}TID13{]}}         &0.732&0.831&0.447&0.033&&0.611&0.702&0.470&0.105&\\ \hline
\multirow{3}{*}{{\bf All}}           & {\bf All {[}LIVE{]}}            &0.958&0.945&0.955&0.961&&0.960&0.961&0.950&0.947&\\ \cline{2-12} 
                                     & {\bf All {[}Multi{]}}           &0.821&0.888&0.852&0.773&&0.883&0.863&0.818&0.900&\\ \cline{2-12} 
                                     & {\bf All {[}TID13{]}}           &0.827&0.866&0.854&0.739&&0.777&0.801&0.853&0.621&\\ \hline
\end{tabular}
\end{table*}


==> Preprint for Arxiv/tab_results_all.tex <==

\begin{table*}[htbp!]
\scriptsize
\centering
\caption{Performance of IQA methods on different databases}
\label{tab_results_databases}
\begin{tabular}{ccccccccccccc}
\hline
               & \textbf{PSNR} & \textbf{PSNR-HA} & \textbf{PSNR-HMA} & \textbf{SSIM} & \textbf{MS-SSIM} & \textbf{CW-SSIM} & \textbf{IW-SSIM} & \textbf{SR-SIM} & \textbf{FSIM} & \textbf{FSIMc} & \textbf{PerSIM} & \textbf{ReSIFT}  \\ \hline
               & \multicolumn{12}{c}{\textbf{Pearson Correlation Coefficicent}}                                                                                                                                                                        \\ \hline
\textbf{LIVE}  & 0.927             &0.953                  &0.958                   &0.945               &0.946                  &0.872                  &0.951                  &0.945                 &0.949               &0.950                &0.955                 &\textbf{0.961}                                 \\ 
\textbf{MULTI} &0.739               &0.801                  &0.821                   &              0.812 & 0.802                 &0.379                  &0.847                  &0.888                 &0.818               & 0.821               & 0.852               &\textbf{0.906}                  \\ \hline

\textbf{}      & \multicolumn{12}{c}{\textbf{Spearman Correlation Coefficient}}                                                                                                                                                                        \\ \hline
\textbf{LIVE}  &0.909               &0.937                 &0.944                   &              0.949 & 0.951                 & 0.902                 & 0.960                 &0.955                 &  0.961          & 0.959              & 0.950                & \textbf{0.962} \\ 
\textbf{MULTI} &0.677               & 0.714                 & 0.742                  &              0.860  &0.836                  & 0.630                 &0.883                  &                0.866               & 0.863               & 0.866                &  0.818             & \textbf{0.887}              \\ \hline
\end{tabular}
\vspace{-4.0mm}
\end{table*}

==> Preprint for Arxiv/tab_results_types.tex <==
\begin{table*}[htbp!]
\scriptsize
\centering
\caption{Performance of best performing IQA methods on different distortion types}
\label{tab_results_types}
\begin{tabular}{c|c|cccc|ccccc}
\hline


\multirow{4}{*}{\bf Distortion Types} & \multirow{4}{*}{\bf Databases} & \multicolumn{4}{c|}{\multirow{2}{*}{\bf Pearson Correlation}}                                                            & \multicolumn{5}{c}{\multirow{2}{*}{\bf Spearman Correlation}}                                                            \\
                  &                   & \multicolumn{4}{l|}{}                                                                             & \multicolumn{5}{l}{}                                                                             \\ \cline{3-11} 
                  &                    & \multirow{2}{*}{\bf PSNR-HMA} & \multirow{2}{*}{\bf SR-SIM} & \multirow{2}{*}{\bf PerSIM}  & \multirow{2}{*}{\bf ReSIFT} & \multirow{2}{*}{\bf IW-SSIM} & \multirow{2}{*}{\bf FSIM} & \multirow{2}{*}{\bf FSIMc} & \multirow{2}{*}{\bf SR-SIM} & \multirow{2}{*}{\bf ReSIFT} \\
                  &                   &                                     &                   &                   &                   &                   &                   &                   &                   &                   \\ \hline

\multirow{3}{*}{{\bf Compression}}   & {\bf Jp2k {[}LIVE{]}}           &\textbf{0.982}&0.957&0.976&0.972&0.979&0.981&\textbf{0.982}&0.972&0.971          \\  
                                     & {\bf Jpeg {[}LIVE{]}}           &\textbf{0.972}&0.950&0.959&0.964&0.960&\textbf{0.962}&\textbf{0.962}&0.954&0.955     \\ 
                                     
                                     & {\bf Blur-Jpeg {[}MULTI{]}}     &0.838&0.904&0.864&\textbf{0.921}&0.869&0.854&0.855&0.862&\textbf{0.886} \\ \hline
\multirow{2}{*}{{\bf Noise}}         & {\bf Wn {[}LIVE{]}}             &0.985&0.974&0.968&\textbf{0.986}&0.982&0.980&0.979&0.983&\textbf{0.984}\\  
                                     & {\bf Blur-Noise {[}MULTI{]}}    &0.803&0.871&0.839&\textbf{0.897}&\textbf{0.893}&0.864&0.869&0.863&0.882\\ \hline
                                     
\multirow{1}{*}{{\bf Communication}} & {\bf FF {[}LIVE{]}}             &\textbf{0.954}&0.943&0.946&0.949&0.967&0.970&\textbf{0.971}&0.966&0.959\\ \hline
                                     
\multirow{3}{*}{{\bf Blur}}          & {\bf GBlur {[}LIVE{]}}          &0.950&0.949&0.967&\textbf{0.971}&\textbf{0.983}&\textbf{0.983}&\textbf{0.983}&0.978&0.979\\  
                                     
                                     & {\bf Blur-Jpeg {[}MULTI{]}}     &0.838&0.904&0.864&\textbf{0.921}&0.869&0.854&0.855&0.862&\textbf{0.886}\\ 
                                     & {\bf Blur-Noise {[}MULTI{]}}    &0.803&0.871&0.839&\textbf{0.897}&\textbf{0.893}&0.864&0.869&0.863&0.882\\ \hline

\end{tabular}
\end{table*}


==> tab_results.tex <==
\begin{table*}[]
\scriptsize
\centering
\caption{Performance of the IQA metrics based on Spearman correlation}
\label{tab_results}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline


\multirow{4}{*}{\bf Distortion Types} & \multirow{4}{*}{\bf Databases} & \multicolumn{5}{c|}{\multirow{2}{*}{\bf Pearson Correlation}}                                                            & \multicolumn{5}{c|}{\multirow{2}{*}{\bf Spearman Correlation}}                                                            \\
                  &                   & \multicolumn{5}{l|}{}                                                                             & \multicolumn{5}{l|}{}                                                                             \\ \cline{3-12} 
                  &                    & \multirow{2}{*}{\bf PSNR-HMA} & \multirow{2}{*}{\bf SR-SIM} & \multirow{2}{*}{\bf PerSIM} & \multirow{2}{*}{\bf SIFT} & \multirow{2}{*}{\bf Proposed} & \multirow{2}{*}{\bf IW-SSIM} & \multirow{2}{*}{\bf FSIM} & \multirow{2}{*}{\bf PerSIM} & \multirow{2}{*}{\bf SIFT} & \multirow{2}{*}{\bf Proposed} \\
                  &                   &                   &                   &                   &                   &                   &                   &                   &                   &                   &                   \\ \hline

\multirow{4}{*}{{\bf Compression}}   & {\bf Jp2k {[}LIVE{]}}           &0.982&0.957&0.976&0.966&0.000&0.979&0.981&0.977&0.959&0.000          \\ \cline{2-12} 
                                     & {\bf Jpeg {[}LIVE{]}}           &0.972&0.950&0.959&0.967&&0.960&0.962&0.958&0.948&       \\ \cline{2-12} 
                                     & {\bf Compression {[}TID13{]}}   &0.969&0.970&0.965&0.906&&0.937&0.960&0.963&0.888& \\ \cline{2-12} 
                                     & {\bf Blur-Jpeg {[}MULTI{]}}     &0.838&0.904&0.864&0.845&&0.869&0.854&0.812&0.893& \\ \hline
\multirow{3}{*}{{\bf Noise}}         & {\bf Wn {[}LIVE{]}}             &0.985&0.974&0.968&0.982&&0.980&0.979&0.991&0.975&\\ \cline{2-12} 
                                     & {\bf Blur-Noise {[}MULTI{]}}    &0.803&0.871&0.839&0.768&&0.893&0.864&0.818&0.903&\\ \cline{2-12} 
                                     & {\bf Noise {[}TID13{]}}         &0.907&0.894&0.903&0.746&&0.856&0.887&0.924&0.721&\\ \hline
\multirow{2}{*}{{\bf Communication}} & {\bf FF {[}LIVE{]}}             &0.954&0.943&0.946&0.946&&0.967&0.970&0.945&0.925&\\ \cline{2-12} 
                                     & {\bf Communication {[}TID13{]}} &0.800&0.905&0.854&0.793&&0.870&0.895&0.865&0.846&\\ \hline
\multirow{4}{*}{{\bf Blur}}          & {\bf GBlur {[}LIVE{]}}          &0.950&0.949&0.967&0.973&&0.983&0.983&0.973&0.961&\\ \cline{2-12} 
                                     & {\bf Blur {[}TID13{]}}          &0.931&0.959&0.935&0.892&&0.932&0.947&0.949&0.857&\\ \cline{2-12} 
                                     & {\bf Blur-Jpeg {[}MULTI{]}}     &0.838&0.904&0.864&0.845&&0.869&0.854&0.812&0.893&\\ \cline{2-12} 
                                     & {\bf Blur-Noise {[}MULTI{]}}    &0.803&0.871&0.839&0.768&&0.893&0.864&0.818&0.903&\\ \hline
{\bf Color}                          & {\bf Color {[}TID13{]}}         &0.814&0.672&0.800&0.663&&0.233&0.240&0.762&0.307&\\ \hline
{\bf Global}                      & {\bf Global {[}TID13{]}}     	   &0.762&0.571&0.585&0.075&&0.452&0.441&0.408&0.104&\\ \hline
{\bf Local}                          & {\bf Local {[}TID13{]}}         &0.732&0.831&0.447&0.033&&0.611&0.702&0.470&0.105&\\ \hline
\multirow{3}{*}{{\bf All}}           & {\bf All {[}LIVE{]}}            &0.958&0.945&0.955&0.961&&0.960&0.961&0.950&0.947&\\ \cline{2-12} 
                                     & {\bf All {[}Multi{]}}           &0.821&0.888&0.852&0.773&&0.883&0.863&0.818&0.900&\\ \cline{2-12} 
                                     & {\bf All {[}TID13{]}}           &0.827&0.866&0.854&0.739&&0.777&0.801&0.853&0.621&\\ \hline
\end{tabular}
\end{table*}

